Adversarial Attacks of Vision Tasks in the Past 10 Years: A Survey

With the advent of Large Vision-Language Models (LVLMs), new attack vectors, such as cognitive bias, prompt injection, and jailbreaking, have emerged. Understanding these attacks promotes system robustness improvement and neural networks demystification. However, existing surveys often target attack taxonomy and lack in-depth analysis like 1) unified insights into adversariality, transferability, and generalization; 2) detailed evaluations framework; 3) motivation-driven attack categorizations; and 4) an integrated perspective on both traditional and LVLM attacks. This article addresses these gaps by offering a thorough summary of traditional and LVLM adversarial attacks, emphasizing their connections and distinctions, and providing actionable insights for future research.

==> Tables/7_LVLM/VLM_methods_techniques.tex <==
\begin{table}
  \caption{Comparison of Techniques Used in LVLM Adversarial Attacks. CIG denotes Conditional Image Generation.}
  \label{tab:VLM_methods_techniques}
  \begin{tabular}{ccccc}
    \toprule
    Methods & Prompt Manipulation & Adversarial Perturbation & CIG & Typography \\
    \midrule
    SASP (2023) \cite{p1}       & \ding{52} &           &           &           \\
    AnyDoor (2024) \cite{p1}    & \ding{52} & \ding{52} &           &           \\
    UMK (2024) \cite{p1}        & \ding{52} & \ding{52} &           &           \\
    BAP (2024) \cite{p1}        & \ding{52} & \ding{52} &           &           \\
    TMM (2024) \cite{p1}        & \ding{52} & \ding{52} &           &           \\
    PPI (2023) \cite{p1}        &           &           &           & \ding{52} \\
    IPI (2023) \cite{p1}        &           &           &           & \ding{52} \\
    FigStep (2023) \cite{p1}    & \ding{52} &           &           & \ding{52} \\
    SGTA (2024) \cite{p1}       & \ding{52} &           &           & \ding{52} \\
    InstructTA (2023) \cite{p1} &           & \ding{52} & \ding{52} &           \\
    CAA (2024) \cite{p1}        & \ding{52} & \ding{52} &           & \ding{52} \\
    MM-SB (2023) \cite{p1}      & \ding{52} &           & \ding{52} & \ding{52} \\
    VRP (2024) \cite{p1}        & \ding{52} &           & \ding{52} & \ding{52} \\
    HADES (2024) \cite{p1}      & \ding{52} & \ding{52} & \ding{52} & \ding{52} \\
  \bottomrule
\end{tabular}
\end{table}
